Definability Results for Top-Down Tree Transducers

We prove that for a given deterministic top-down transducer with look-ahead it is decidable whether or not its translation is definable (1)~by a linear top-down tree transducer or (2)~by a tree homomorphism. We present algorithms that construct equivalent such transducers if they exist.

==> conclusion.tex <==
\section{Conclusion}

==> introduction.tex <==
	\section{Introduction}
% Tree transformations are a fundamental aspect of XML database theory and can oftentimes be realized by \emph{deterministic  top-down tree transducers}.\cite{10.5555/1941946, DBLP:conf/pods/LemayMN10, DBLP:journals/jcss/EngelfrietMS09, DBLP:conf/dbpl/ManethN99, DBLP:journals/iandc/MartensNG08, DBLP:journals/jcss/MartensN07} 
A top-down transducer is a finite state
 device that processes an input tree and generates an output tree in a parallel top-down fashion. A more expressive but 
 at the same time more complex model for realizing tree transformations are \emph{deterministic  top-down tree transducers with regular look-ahead}. Such devices consists of a  top-down tree transducer and a \emph{bottom-up tree automaton}
 and  process an input tree in two phases:
 First the input tree is relabeled by the bottom-up automaton.
 In the second phase the top-down tree transducer processes the relabeled tree making use of the information the relabeled nodes provide about
 the respective subtees rooted at those nodes.
 
 Due to the complexity of top-down tree transducers with regular look-ahead, a natural question is: 
 given a top-down tree transducers with regular look-ahead when can its translation be realized by a
  top-down tree transducer. This question has been answered in \cite{DBLP:journals/tcs/EngelfrietMS16}, however the described method requires prior knowledge about \emph{difference  trees} and \emph{difference bounds}, i.e., knowledge about how different look-ahead states affect the translation. Answering this question  does not require any 
  prior knowledge if we restrict ourselves to particular subclasses of transducers. More precisely, in \cite{DBLP:conf/icalp/ManethS20} it has been proven that
   it is decidable whether or not for a given  uniform-copying linear (linear) 
  top-down tree transducers with regular look-ahead an equivalent uniform-copying linear (linear) top-down tree transducer  exists.
    A \emph{uniform-copying} top-down tree transducer (with look- ahead) is a transducer  in which all copies of an input subtree 
  are processed  by the same state while a\emph{linear} top-down tree transducer (with look- ahead) is not allowed to copy input subtrees at all.
  
  In this paper we extend the results of \cite{DBLP:conf/icalp/ManethS20}.
 In particular we show that it is decidable whether or not for a given top-down tree transducers with regular look-ahead
 (1) an equivalent linear top-down tree transducer or (2) an equivalent \emph{homomorphism}, i.e., a single state   top-down tree transducers,  exists and if so how to construct the corresponding transducer.
  Note that homomorphism are a special case of uniform-copying transducers.
  
  Transforming  transducers with regular look-ahead into these simpler forms allows us to implement the corresponding tree translations 
  with less resources and hence more efficiently. Additionally we can make use of the special properties this particular classes of transducers have. 
  For instance  linear tree transducers preserve regularity\cite[Corollary~3.11]{DBLP:journals/mst/Engelfriet77}.
  This property is particularly useful when considering  \emph{typechecking}, i.e., the question whether  given a tree transducer $M$
  a set of input trees $\mathcal{T}_{in}$ and a set of trees $\mathcal{T}_{out}$ does $M$ produce an output
  tree specified according to $\mathcal{T}_{out}$ for all inputs in $\mathcal{T}_{in}$?
  As  linear tree transducers preserve regularity this question can be answered using the simpler \emph{forward type inference} approach instead
  of the more complicated \emph{backward type inference} method.
  \cite{10.5555/1941946}\\
   As a side  note we remark that  similar to  \cite{DBLP:journals/tcs/EngelfrietMS16} and \cite{DBLP:conf/icalp/ManethS20} 
we make extensive use
  of the \emph{canonical earliest normal form} showing how versatile this normal form is. 

